Creating and Querying Data Cubes in Python using pyCube

Data cubes are used for analyzing large data sets usually contained in data warehouses. The most popular data cube tools use graphical user interfaces (GUI) to do the data analysis. Traditionally this was fine since data analysts were not expected to be technical people. However, in the subsequent decades the data landscape changed dramatically requiring companies to employ large teams of highly technical data scientists in order to manage and use the ever increasing amount of data. These data scientists generally use tools like Python, interactive notebooks, pandas, etc. while modern data cube tools are still GUI based. This paper proposes a Python-based data cube tool called pyCube. pyCube is able to semi-automatically create data cubes for data stored in an RDBMS and manages the data cube metadata. pyCube's programmatic interface enables data scientist to query data cubes by specifying the expected metadata of the result. pyCube is experimentally evaluated on Star Schema Benchmark (SSB). The results show that pyCube vastly outperforms different implementations of SSB queries in pandas in both runtime and memory while being easier to read and write.

==> algorithms/cube_inference.tex <==
\begin{algorithm}
    \caption{Inferring the Cube}
    \label{alg:inf_cube}
    \begin{algorithmic}[1]
        \State factTable = \Call{FindFactTable}{ }\label{algl:findFactTable}
        \State bottomLevels = \Call{FindBottomLevels}{factTable}\label{algl:findBottomLevels}
        \State allLevels = []\label{algl:allLevels}
        \State levelAttributes = []\label{algl:levelAttributes}
        \ForAll{level $\in$ bottomLevels}\label{algl:forloop}
            \State levels = []\label{algl:levels}
            \State level\_attributes = []\label{algl:level_attributes}
            \State currentLevel = level\label{algl:currentLevel}
            \While{True}\label{algl:whileloop}
                \If{currentLevel is not Null}
                    \State levels.append(currentLevel)\label{algl:append}
                    \State c = \Call{FindNonKeyColumns}{currentLevel}\label{algl:findNonKeyColumns}
                    \If{len(c) > 1}\label{algl:ifLen}
                        \State attributes = \Call{FindLevelAttributes}{c}\label{algl:removeLevelMember}
                        \State level\_attributes.append(attributes)
                    \EndIf
                \Else
                    \State \textbf{break}
                \EndIf
                \State currentLevel = \Call{FindNextTable}{currentLevel}\label{algl:findNextTable}
            \EndWhile
            \State allLevels.append(levels)
            \State levelAttributes.append(level\_attributes)
        \EndFor
        \State measures = \Call{FindMeasures}{factTable}\label{algl:findMeasures}
        \State \Call{AddToGraph}{levels, levelAttributes, measures}\label{algl:addToGraph}
    \end{algorithmic}
\end{algorithm}


==> definitions/axis.tex <==
\begin{definition}[Axis]\label{def:axis}
    Let $ds = (LS, \preceq)$ be a dimension schema, and let $d = (LM, R)$ be a dimension instance of $ds$.
    An \emph{axis} $ax = (d, \ell, a, lm)$ is a 4-tuple, where $d$ is a dimension instance, $\ell = (k, A)\in LS$ is a level schema, $a\in A$ is an attribute on $\ell$ and $lm$ is a list of level members from $LM_\ell$.
\end{definition}


==> definitions/data_cube_instance.tex <==
\begin{definition}[Data Cube Instance]\label{def:data_cube_instance}
    Let $cs = (DS, MS)$ be a data cube schema, $D_I$ be a set of dimension instances with exactly one dimension instance for each dimension schema in $DS$ and $LM_i$ be the set of level members in the i\textsuperscript{th} dimension instance.
    Furthermore let $B_{D_I} = \bigtimes_{j = 1}^{|D_I|}LM_{j}$ be the cartesian product of the level members across all dimension instances, and let $B_{MS} = (\mathbb{R}\cup\{\bot\})^{|MS|}$ be the numerical values of the measures where $\bot$ denotes no value.
    A \emph{data cube instance} $\cubeinstance : B_{D_I}\rightarrow B_{MS}$ is a function that maps combinations of level members from $B_{D_I}$ to the numerical values of the measures from $B_{MS}$.
\end{definition}


==> definitions/data_cube_schema.tex <==
\begin{definition}[Data Cube Schema]
    A \emph{data cube schema} $cs = (DS, MS)$ is a tuple, where $DS$ is a set of dimension schemas, and $MS$ is a set of measure schemas.
\end{definition}


==> definitions/data_cube_view.tex <==
\begin{definition}[Data Cube View]\label{def:data_cube_view}
    A data cube view $v = (AX, \\ MS_v, p, c)$ is a 4-tuple where $AX = \{ax_0, ax_1,\dots,ax_n\}$ and $MS_v = \{ms_1, ms_2,\dots, ms_m\}$ are ordered sets of axes and measure schemas respectively, $p$ is a predicate tree and \cubeinstance is the corresponding data cube instance.
\end{definition}


==> definitions/dimension_instance.tex <==
\begin{definition}[Dimension Instance]
    Let $ds = (LS, \preceq)$ be a dimension schema and let $LI$ be an ordered set of level instances with exactly one level instance for each level schema in LS.
    A \emph{dimension instance} $d = (LM, R)$ of $ds$ is a tuple, where 
    \begin{enumerate}
        \item $LM = \{LM_1, LM_2,\dots, LM_{|LI|}\}$ is an ordered set of disjoint multisets of attribute values for each level instance $li\in LI$ called \emph{level members}, and 
        \item $R = \{R_1,R_2,\dots R_{|LS|}\}$ is an ordered set of sets of \emph{roll-up} functions, one set for each set of level members, such that if $r(lm_i) = lm_j$ for some $r\in R_i$ then $ls_i\preceq ls_j$, for every $lm_i\in LM_i$ and $lm_j\in LM_j$, together with their associated level schemas $ls_i$ and $ls_j$, where $1\leq i, j\leq |LS|$.
    \end{enumerate}
\end{definition}


==> definitions/dimension_schema.tex <==
\begin{definition}[Dimension Schema]
    A \emph{dimension schema} $ds = (LS, \preceq)$ is a tuple, where $LS$ is a set of level schemas including the level schema $ALL_{ds} = (\{all\}, \{all\})$ and $\preceq$ is a partial order on the level schemas $ls\in LS$.
\end{definition}


==> definitions/level_instance.tex <==
\begin{definition}[Level Instance]
    Let $ls = (k, A)$ be a level schema.
    %A level instance of $ls$ is a function that maps each attribute $a\in A$ to a multiset of values in the domain of $a$.
    A \emph{level instance} of $ls$ is a function that maps from values of $k$ to tuples in $dom(a_1) \times \cdots \times dom(a_n)$
    for $a_1, \ldots, a_n \in A$ where $dom(a_i)$ denotes the domain of $a_i$, i.e., the set of possible values for $a_i$.
\end{definition}



==> definitions/level_schema.tex <==
\begin{definition}[Level Schema]
    A \emph{level schema} $ls = (k, A)$ is a tuple, where $k\subseteq A$ is the \emph{level key} consisting of one or more attributes, and $A$ is a set of attributes.
\end{definition}


==> definitions/measure.tex <==
\begin{definition}[Measure Schema]\label{def:measure_schema}
    A \emph{measure schema} $ms = (a, \emph{agg})$ is a tuple, where $a$ is an attribute with values in $\mathbb{R}$ and $\emph{agg}$ is an aggregate function which takes in a multiset of real numbers and returns a value $r\in\mathbb{R}$.
\end{definition}


==> definitions/predicate.tex <==
\begin{definition}[Predicate]\label{def:predicate}
   Let $ls = (k, A)$ be a level schema and $a \in A$ be an attribute. Let $\omega \in \{<, \leq, =, \neq, \geq, >\}$ be a numeric operator. Let $lit$ be a literal.  
  An expression of the form  \emph{true}, \emph{false}, or $a$ $\omega$ $lit$ is a predicate. If $p_1,p_2$ are predicates, then $(p_1)$, %$\neg p_1$, 
    $p_1 \wedge p_2$, and $p_1 \vee p_2$ are predicates. The evaluation order is defined by the standard operator bindings.
\end{definition}


==> figures/laptop/sf1/mem.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width  = 0.8*\textwidth,
        height = 4cm,
        major x tick style = transparent,
        ybar=1.2pt,
        bar width=4pt,
        ymajorgrids = true,
        ylabel = {Memory (GB)},
        y label style = {font=\footnotesize,at={(-0.06,0.5)}},
        symbolic x coords={Q11,Q12,Q13,Q21,Q22,Q23,Q31,Q32,Q33,Q34,Q41,Q42,Q43},
        xtick = data,
        scaled y ticks = false,
        ymin=0
    ]
        \addplot[style={bblue,fill=bblue,mark=none}]
coordinates {(Q11, 0.104) (Q12, 0.102) (Q13, 0.102) (Q21, 0.104) (Q22, 0.103) (Q23, 0.105) (Q31, 0.103) (Q32, 0.105) (Q33, 0.103) (Q34, 0.104) (Q41, 0.103) (Q42, 0.104) (Q43, 0.104) };
        \addplot[style={rred,fill=rred,mark=none}]
coordinates {(Q11, 10.313) (Q12, 8.671) (Q13, 10.313) (Q21, 21.372) (Q22, 20.527) (Q23, 20.527) (Q31, 7.726) (Q32, 6.224) (Q33, 4.677) (Q34, 4.958) (Q41, 12.501) (Q42, 11.962) (Q43, 12.173) };
        \addplot[style={ggreen,fill=ggreen,mark=none}]
coordinates {(Q11, 2.093) (Q12, 2.093) (Q13, 2.234) (Q21, 4.114) (Q22, 3.834) (Q23, 3.833) (Q31, 4.443) (Q32, 4.208) (Q33, 3.505) (Q34, 3.693) (Q41, 6.987) (Q42, 7.177) (Q43, 7.201) };
        \addplot[style={ppurple,fill=ppurple,mark=none}]
coordinates {(Q11, 2.06) (Q12, 2.093) (Q13, 2.294) (Q21, 3.267) (Q22, 2.794) (Q23, 2.793) (Q31, 3.98) (Q32, 3.981) (Q33, 2.792) (Q34, 3.281) (Q41, 4.543) (Q42, 4.907) (Q43, 4.908) };
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q11) at (axis cs:Q11, 0.104) {0.104};
        \draw[->,style={bblue},bend left] (Q11.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q11, 0.104.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q12) at (axis cs:Q12, 0.102) {0.102};
        \draw[->,style={bblue},bend left] (Q12.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q12, 0.102.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q13) at (axis cs:Q13, 0.102) {0.102};
        \draw[->,style={bblue},bend left] (Q13.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q13, 0.102.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q21) at (axis cs:Q21, 0.104) {0.104};
        \draw[->,style={bblue},bend left] (Q21.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q21, 0.104.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q22) at (axis cs:Q22, 0.103) {0.103};
        \draw[->,style={bblue},bend left] (Q22.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q22, 0.103.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q23) at (axis cs:Q23, 0.105) {0.105};
        \draw[->,style={bblue},bend left] (Q23.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q23, 0.105.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q31) at (axis cs:Q31, 0.103) {0.103};
        \draw[->,style={bblue},bend left] (Q31.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q31, 0.103.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q32) at (axis cs:Q32, 0.105) {0.105};
        \draw[->,style={bblue},bend left] (Q32.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q32, 0.105.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q33) at (axis cs:Q33, 0.103) {0.103};
        \draw[->,style={bblue},bend left] (Q33.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q33, 0.103.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q34) at (axis cs:Q34, 0.104) {0.104};
        \draw[->,style={bblue},bend left] (Q34.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q34, 0.104.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q41) at (axis cs:Q41, 0.103) {0.103};
        \draw[->,style={bblue},bend left] (Q41.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q41, 0.103.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q42) at (axis cs:Q42, 0.104) {0.104};
        \draw[->,style={bblue},bend left] (Q42.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q42, 0.104.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q43) at (axis cs:Q43, 0.104) {0.104};
        \draw[->,style={bblue},bend left] (Q43.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q43, 0.104.north);
    \end{axis}
\end{tikzpicture}



==> figures/laptop/sf10/mem.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width  = 0.8*\textwidth,
        height = 4cm,
        major x tick style = transparent,
        ybar=1.2pt,
        bar width=4pt,
        ymajorgrids = true,
        ylabel = {Memory (GB)},
        y label style = {font=\footnotesize,at={(-0.05,0.5)}},
        symbolic x coords={Q11,Q12,Q13,Q21,Q22,Q23,Q31,Q32,Q33,Q34,Q41,Q42,Q43},
        xtick = data,
        scaled y ticks = false,
        ymin=0
    ]
        \addplot[style={bblue,fill=bblue,mark=none}]
coordinates {(Q11, 0.101) (Q12, 0.101) (Q13, 0.101) (Q21, 0.098) (Q22, 0.098) (Q23, 0.099) (Q31, 0.098) (Q32, 0.098) (Q33, 0.098) (Q34, 0.098) (Q41, 0.098) (Q42, 0.098) (Q43, 0.099)};
        \addplot[style={rred,fill=rred,mark=none}]
coordinates {};
        \addplot[style={ggreen,fill=ggreen,mark=none}]
coordinates {(Q11, 19.934) (Q12, 19.935) (Q13, 20.829) };
        \addplot[style={ppurple,fill=ppurple,mark=none}]
coordinates {(Q11, 19.924) (Q12, 19.934) (Q13, 22.022) };
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q11) at (axis cs:Q11, 0.101) {0.101};
        \draw[->,style={bblue},bend left] (Q11.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q11, 0.101.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q12) at (axis cs:Q12, 0.101) {0.101};
        \draw[->,style={bblue},bend left] (Q12.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q12, 0.101.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q13) at (axis cs:Q13, 0.101) {0.101};
        \draw[->,style={bblue},bend left] (Q13.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q13, 0.101.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q21) at (axis cs:Q21, 0.099) {0.098};
        \draw[->,style={bblue},bend left] (Q21.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q21, 0.099.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q22) at (axis cs:Q22, 0.099) {0.098};
        \draw[->,style={bblue},bend left] (Q22.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q22, 0.099.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q23) at (axis cs:Q23, 0.098) {0.099};
        \draw[->,style={bblue},bend left] (Q23.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q23, 0.098.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q31) at (axis cs:Q31, 0.098) {0.098};
        \draw[->,style={bblue},bend left] (Q31.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q31, 0.098.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q32) at (axis cs:Q32, 0.099) {0.098};
        \draw[->,style={bblue},bend left] (Q32.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q32, 0.099.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q33) at (axis cs:Q33, 0.098) {0.098};
        \draw[->,style={bblue},bend left] (Q33.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q33, 0.098.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q34) at (axis cs:Q34, 0.098) {0.098};
        \draw[->,style={bblue},bend left] (Q34.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q34, 0.098.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q41) at (axis cs:Q41, 0.098) {0.098};
        \draw[->,style={bblue},bend left] (Q41.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q41, 0.098.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q42) at (axis cs:Q42, 0.098) {0.098};
        \draw[->,style={bblue},bend left] (Q42.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q42, 0.098.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q43) at (axis cs:Q43, 0.099) {0.099};
        \draw[->,style={bblue},bend left] (Q43.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q43, 0.099.north);
    \end{axis}
\end{tikzpicture}


==> figures/laptop/sf2/mem.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width  = 0.8*\textwidth,
        height = 4cm,
        major x tick style = transparent,
        ybar=1.2pt,
        bar width=4pt,
        ymajorgrids = true,
        ylabel = {Memory (GB)},
        y label style = {font=\footnotesize,at={(-0.05,0.5)}},
        symbolic x coords={Q11,Q12,Q13,Q21,Q22,Q23,Q31,Q32,Q33,Q34,Q41,Q42,Q43},
        xtick = data,
        scaled y ticks = false,
        ymin=0
    ]
        \addplot[style={bblue,fill=bblue,mark=none}]
coordinates {(Q11, 0.097) (Q12, 0.099) (Q13, 0.097) (Q21, 0.098) (Q22, 0.098) (Q23, 0.098) (Q31, 0.098) (Q32, 0.098) (Q33, 0.098) (Q34, 0.098) (Q41, 0.098) (Q42, 0.098) (Q43, 0.099) };
        \addplot[style={rred,fill=rred,mark=none}]
coordinates {(Q11, 20.529) (Q12, 17.248) (Q13, 20.529) (Q31, 15.328) (Q32, 12.329) (Q33, 9.235) (Q34, 9.798) (Q41, 24.95) (Q42, 23.918) (Q43, 24.388) };
        \addplot[style={ggreen,fill=ggreen,mark=none}]
coordinates {(Q11, 3.778) (Q12, 3.776) (Q13, 4.239) (Q21, 8.018) (Q22, 7.454) (Q23, 7.455) (Q31, 8.769) (Q32, 8.298) (Q33, 6.892) (Q34, 7.267) (Q41, 13.889) (Q42, 14.263) (Q43, 14.358) };
        \addplot[style={ppurple,fill=ppurple,mark=none}]
coordinates {(Q11, 3.812) (Q12, 3.806) (Q13, 4.48) (Q21, 6.427) (Q22, 5.477) (Q23, 5.478) (Q31, 7.851) (Q32, 7.851) (Q33, 5.477) (Q34, 6.425) (Q41, 8.974) (Q42, 9.705) (Q43, 9.706) };
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q11) at (axis cs:Q11, 0.097) {0.097};
        \draw[->,style={bblue},bend left] (Q11.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q11, 0.097.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q12) at (axis cs:Q12, 0.099) {0.099};
        \draw[->,style={bblue},bend left] (Q12.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q12, 0.099.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q13) at (axis cs:Q13, 0.097) {0.097};
        \draw[->,style={bblue},bend left] (Q13.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q13, 0.097.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q21) at (axis cs:Q21, 0.098) {0.098};
        \draw[->,style={bblue},bend left] (Q21.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q21, 0.098.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q22) at (axis cs:Q22, 0.098) {0.098};
        \draw[->,style={bblue},bend left] (Q22.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q22, 0.098.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q23) at (axis cs:Q23, 0.098) {0.098};
        \draw[->,style={bblue},bend left] (Q23.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q23, 0.098.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q31) at (axis cs:Q31, 0.098) {0.098};
        \draw[->,style={bblue},bend left] (Q31.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q31, 0.098.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q32) at (axis cs:Q32, 0.098) {0.098};
        \draw[->,style={bblue},bend left] (Q32.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q32, 0.098.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q33) at (axis cs:Q33, 0.098) {0.098};
        \draw[->,style={bblue},bend left] (Q33.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q33, 0.098.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q34) at (axis cs:Q34, 0.098) {0.098};
        \draw[->,style={bblue},bend left] (Q34.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q34, 0.098.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q41) at (axis cs:Q41, 0.098) {0.098};
        \draw[->,style={bblue},bend left] (Q41.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q41, 0.098.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q42) at (axis cs:Q42, 0.098) {0.098};
        \draw[->,style={bblue},bend left] (Q42.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q42, 0.098.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q43) at (axis cs:Q43, 0.099) {0.099};
        \draw[->,style={bblue},bend left] (Q43.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q43, 0.099.north);
    \end{axis}
\end{tikzpicture}


==> figures/laptop/sf5/mem.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width  = 0.8*\textwidth,
        height = 4cm,
        major x tick style = transparent,
        ybar=1.2pt,
        bar width=4pt,
        ymajorgrids = true,
        ylabel = {Memory (GB)},
        y label style = {font=\footnotesize,at={(-0.05,0.5)}},
        symbolic x coords={Q11,Q12,Q13,Q21,Q22,Q23,Q31,Q32,Q33,Q34,Q41,Q42,Q43},
        xtick = data,
        scaled y ticks = false,
        ymin=0
    ]
        \addplot[style={bblue,fill=bblue,mark=none}]
coordinates {(Q11, 0.097) (Q12, 0.097) (Q13, 0.097) (Q21, 0.099) (Q22, 0.099) (Q23, 0.098) (Q31, 0.098) (Q32, 0.099) (Q33, 0.098) (Q34, 0.098) (Q41, 0.098) (Q42, 0.098) (Q43, 0.099) };
        \addplot[style={rred,fill=rred,mark=none}]
coordinates {};
        \addplot[style={ggreen,fill=ggreen,mark=none}]
coordinates {(Q11, 10.046) (Q12, 10.046) (Q13, 10.496) (Q21, 19.888) (Q22, 18.483) (Q23, 18.484) (Q32, 20.593) (Q33, 17.077) (Q34, 18.014) };
        \addplot[style={ppurple,fill=ppurple,mark=none}]
coordinates {(Q11, 10.01) (Q12, 10.044) (Q13, 11.059) (Q21, 16.15) (Q22, 13.551) (Q23, 13.552) (Q31, 19.487) (Q32, 19.487) (Q33, 13.551) (Q34, 16.15) };
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q11) at (axis cs:Q11, 0.097) {0.097};
        \draw[->,style={bblue},bend left] (Q11.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q11, 0.097.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q12) at (axis cs:Q12, 0.097) {0.097};
        \draw[->,style={bblue},bend left] (Q12.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q12, 0.097.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q13) at (axis cs:Q13, 0.097) {0.097};
        \draw[->,style={bblue},bend left] (Q13.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q13, 0.097.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q21) at (axis cs:Q21, 0.099) {0.099};
        \draw[->,style={bblue},bend left] (Q21.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q21, 0.099.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q22) at (axis cs:Q22, 0.099) {0.099};
        \draw[->,style={bblue},bend left] (Q22.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q22, 0.099.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q23) at (axis cs:Q23, 0.098) {0.098};
        \draw[->,style={bblue},bend left] (Q23.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q23, 0.098.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q31) at (axis cs:Q31, 0.098) {0.098};
        \draw[->,style={bblue},bend left] (Q31.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q31, 0.098.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q32) at (axis cs:Q32, 0.099) {0.099};
        \draw[->,style={bblue},bend left] (Q32.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q32, 0.099.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q33) at (axis cs:Q33, 0.098) {0.098};
        \draw[->,style={bblue},bend left] (Q33.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q33, 0.098.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q34) at (axis cs:Q34, 0.098) {0.098};
        \draw[->,style={bblue},bend left] (Q34.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q34, 0.098.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q41) at (axis cs:Q41, 0.098) {0.098};
        \draw[->,style={bblue},bend left] (Q41.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q41, 0.098.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q42) at (axis cs:Q42, 0.098) {0.098};
        \draw[->,style={bblue},bend left] (Q42.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q42, 0.098.north);
        \node[above left,rotate=15,yshift=.51cm,xshift=2pt,style={bblue}] (Q43) at (axis cs:Q43, 0.099) {0.099};
        \draw[->,style={bblue},bend left] (Q43.south) to[xshift=-8pt,yshift=2pt] (axis cs:Q43, 0.099.north);
    \end{axis}
\end{tikzpicture}


==> figures/snowflake_schema.tex <==
\begin{figure*}
  \resizebox{\linewidth}{50em}{
    \begin{tikzpicture}
      \node (sales) at (-3,0) {
        \begin{tabular}{|c|c|c|c|c|c|}
        \hline
        \multicolumn{6}{|c|}{Sales} \\
        \hline
        \hline
        supplier\_id & store\_id & product\_id & sale\_date\_id & total\_sales\_price & unit\_sales \\
        \hline
        1221 & 4623 & 9012 & 2646 & 396 & 4 \\
        \hline
        \end{tabular}
      };

      \node (supplier_name) at (-6,2) {
        \begin{tabular}{|c|c|c|}
        \hline
        \multicolumn{3}{|c|}{name} \\
        \hline
        \hline
        supplier\_id & name & nation\_id \\
        \hline
        1221 & Clothing Brand 1 & 1598 \\
        \hline
        \end{tabular}
      };

      \node (supplier_nation) at (-6,4) {
        \begin{tabular}{|c|c|c|}
        \hline
        \multicolumn{3}{|c|}{nation} \\
        \hline
        \hline
        nation\_id & nation & continent\_id \\
        \hline
        1598 & Denmark & 1991 \\
        \hline
        \end{tabular}
      };

      \node (supplier_continent) at (-6,6) {
        \begin{tabular}{|c|c|}
        \hline
        \multicolumn{2}{|c|}{continent} \\
        \hline
        \hline
        continent\_id & continent \\
        \hline
        1991 & Europe \\
        \hline
        \end{tabular}
      };

      \node (store) at (1.4,2) {
        \begin{tabular}{|c|c|c|c|}
        \hline
        \multicolumn{4}{|c|}{address} \\
        \hline
        \hline
        store\_id & address & size & city\_id \\
        \hline
        4623 & Jyllandsgade 1 & 500 sqm & 4892 \\
        \hline
        \end{tabular}
      };

      \node (store_city) at (1.4,4) {
        \begin{tabular}{|c|c|c|}
        \hline
        \multicolumn{3}{|c|}{city} \\
        \hline
        \hline
        city\_id & city & county\_id \\
        \hline
        4892 & Aalborg & 4921 \\
        \hline
        \end{tabular}
      };

      \node (store_county) at (1.4,6) {
        \begin{tabular}{|c|c|}
        \hline
        \multicolumn{2}{|c|}{county} \\
        \hline
        \hline
        county\_id & county \\
        \hline
        4921 & North Jutland Region \\
        \hline
        \end{tabular}
      };

      \node (product) at (-4.5,-2.5) {
        \begin{tabular}{|c|c|c|}
        \hline
        \multicolumn{3}{|c|}{name} \\
        \hline
        \hline
        product\_id & name & category\_id \\
        \hline
        9012 & Clothing Item 1 & 10234 \\
        \hline
        \end{tabular}
      };

      \node (product_category) at (-5.5,-4.5) {
        \begin{tabular}{|c|c|}
        \hline
        \multicolumn{2}{|c|}{category} \\
        \hline
        \hline
        category\_id & category \\
        \hline
        10234 & Blouse  \\
        \hline
        \end{tabular}
      };

      \node (day) at (3,-2.5) {
        \begin{tabular}{|c|c|c|}
        \hline
        \multicolumn{3}{|c|}{day} \\
        \hline
        \hline
        day\_id & day & month\_id \\
        \hline
        2646 & 7 & 2801 \\
        \hline
        \end{tabular}
      };

      \node (month) at (3,-4.5) {
        \begin{tabular}{|c|c|c|}
        \hline
        \multicolumn{3}{|c|}{month} \\
        \hline
        \hline
        month\_id & month & year\_id \\
        \hline
        2801 & January & 2920 \\
        2802 & February & 2920 \\
        2701 & January & 2919 \\
        \hline
        \end{tabular}
      };

      \node (year) at (3,-7) {
        \begin{tabular}{|c|c|}
        \hline
        \multicolumn{2}{|c|}{year} \\
        \hline
        \hline
        year\_id & year \\
        \hline
        2920 & 2023 \\
        2919 & 2022 \\
        \hline
        \end{tabular}
      };


        \draw[->] (sales.north) to (supplier_name.south);
        \draw[->] (supplier_name.north) to (supplier_nation.south);
        \draw[->] (supplier_nation.north) to (supplier_continent.south);

        \draw[->] (sales.north) to (store.south);
        \draw[->] (store.north) to (store_city.south);
        \draw[->] (store_city.north) to (store_county.south);

        \draw[->] (sales.south) to (product.north);
        \draw[->] (product.south) to (product_category.north);

        \draw[->] (sales.south) to (day.north);
        \draw[->] (day.south) to (month.north);
        \draw[->] (month.south) to (year.north);
    \end{tikzpicture}
  }
  \Description{A schema showing the relational structure of the company's database}
  \caption{The snowflake schema for salesdb and some sample data}
  \label{fig:salesdb_snowflake}
\end{figure*}


==> listings/adding_days_in_june.tex <==
\begin{lstlisting}[caption={Drilling down on the Date dimension},label={lst:change_days}]
c2 = c1.columns(sales_cube.Date.Year["2020"].June
                .children())
\end{lstlisting}


==> listings/adding_product_categories.tex <==
\begin{lstlisting}[caption={Aggregating the products up to the product category},label={lst:change_product}]
c1 = c.rows(sales_cube.Store.Address.members())
\end{lstlisting}


==> listings/adding_products.tex <==
\begin{lstlisting}[caption={Adding products on rows},label={lst:cubecolrows}]
c = sales_cube
        .columns(sales_cube.Date.Year["2020"].children())
        .rows(sales_cube.Product.Name.members())
\end{lstlisting}


==> listings/adding_stores.tex <==
\begin{lstlisting}[caption={Adding stores on pages},label={lst:cubecolrowpages}]
c = sales_cube
        .columns(sales_cube.Date.Year["2020"].children())
        .rows(sales_cube.Product.Category.members())
        .pages(sales_cube.Store.City.members())
\end{lstlisting}


==> listings/change_measure.tex <==
\begin{lstlisting}[caption={Using another measure without changing the default measure},label={lst:measures_method}]
sales_cube.columns(sales_cube.Date.Year["2020"].children())
          .measures(sales_cube.UnitSales)
\end{lstlisting}


==> listings/columns_months_in_2020.tex <==
\begin{lstlisting}[caption={Grouping the cube by the months in 2020},label={lst:colmonth2020}]
c_2020 = sales_cube.columns(sales_cube.Date.Year["2020"]
                            .children())
\end{lstlisting}


==> listings/columns_months_in_2020_result.tex <==
\begin{lstlisting}[caption={The content of the cells when grouped by months in 2020},label={lst:dataframe}]
 J    F    M    A    M    J    J    A    S    O    N    D
7547 6597 8447 7296 9056 5135 1638 2756 1273 9995 1990 2880
\end{lstlisting}


==> listings/config_postgres_engine.tex <==
\begin{lstlisting}[caption={Configuring the postgres engine},label={lst:configuration}]
postgres_engine = pyCube.engines.postgres(
    dbname="salesdb", 
    user="helle", 
    password="password123", 
    host="127.0.0.1", 
    port="5432"
    )
\end{lstlisting}



==> listings/conversion_example.tex <==
\begin{lstlisting}[caption={Manipulating a cube with representational methods},label={lst:conv_cube}]
c = base_cube.columns(base_cube.Date.Year._2020.children())
             .rows(base_cube.Product.Category.members())
             .where(base_cube.Supplier.Nation == "Denmark"
                    base_cube.Date.Day <= 7)
\end{lstlisting}


==> listings/conversion_example1.tex <==
\begin{lstlisting}[caption={Conversion example},label={lst:conversion_example1}]
c = cube.columns(base_cube.Date.Year["2020"].children())
        .rows(base_cube.Product.Category.members())
        .where(base_cube.Supplier.Nation == "Denmark"
               base_cube.Date.Day <= 7)
\end{lstlisting}


==> listings/create_session.tex <==
\begin{lstlisting}[caption={Creating a session},label={lst:create_session}]
session = pyCube.create_session(engine=postgres_engine)
\end{lstlisting}


==> listings/data_structure_definition.tex <==
\begin{minipage}{\linewidth}
\begin{lstlisting}[label={lst:dsd},caption={The DataStructureDefinition produced by running Algorithm~\protect\ref{alg:inf_cube} on the running example}]
eg:salesdb_snowflake_dsd a qb:DataStructureDefinition ;
    qb:component [ qb4o:level eg:supplier_name ],
        [ qb4o:level eg:store_address ],
        [ qb4o:level eg:product_name ],
        [ qb4o:level eg:date_day ],
        [ qb:measure eg:unit_sales ;
            qb4o:hasAggregateFunction qb4o:sum ],
        [ qb:measure eg:total_sales_price ;
            qb4o:hasAggregateFunction qb4o:sum ] .
\end{lstlisting}
\end{minipage}


==> listings/import.tex <==
\begin{lstlisting}[caption={Importing \frameworkname},label={lst:import}]
import pyCube
\end{lstlisting}


==> listings/limit_first_week.tex <==
\begin{lstlisting}[caption={Limit results to first week in month},label={lst:limit_first_week}]
c = sales_cube
        .columns(sales_cube.Date.Year["2020"].children())
        .rows(sales_cube.Product.Category.members())
        .pages(sales_cube.Store.City.members())
        .where(sales_cube.Supplier.Nation == "Denmark" &
               sales_cube.Date.Day <= 7)
\end{lstlisting}


==> listings/list_cubes.tex <==
\begin{lstlisting}[caption={Listing the available views},label={lst:cubes}]
session.views
\end{lstlisting}



==> listings/list_dimensions.tex <==
\begin{lstlisting}[caption={Listing the available dimension schemas},label={lst:show_dimensions}]
sales_view.dimensions()
\end{lstlisting}


==> listings/list_hierarchies.tex <==
\begin{lstlisting}[caption={Listing the hierarchies of the \inlinecode{Date} dimension schema},label={lst:show_hierarchy}]
sales_view.Date.hierarchies()
\end{lstlisting}


==> listings/list_measures.tex <==
\begin{lstlisting}[caption={Listing the available measure schemas},label={lst:show_measures}]
sales_view.measures()
\end{lstlisting}


==> listings/load_cube.tex <==
\begin{lstlisting}[caption={Saving the view in a variable},label={lst:load_cube}]
sales_view = session.Sales
\end{lstlisting}


==> listings/months_in_2020.tex <==
\begin{lstlisting}[label={lst:children},caption={Grouping the cube by the months in 2020}]
c_2020 = sales_cube.columns([
    sales_cube.Date.Year["2020"].January, 
    sales_cube.Date.Year["2020"].February, 
    sales_cube.Date.Year["2020"].March, 
    sales_cube.Date.Year["2020"].April, 
    sales_cube.Date.Year["2020"].May, 
    sales_cube.Date.Year["2020"].June, 
    sales_cube.Date.Year["2020"].July, 
    sales_cube.Date.Year["2020"].August, 
    sales_cube.Date.Year["2020"].September, 
    sales_cube.Date.Year["2020"].October, 
    sales_cube.Date.Year["2020"].November, 
    sales_cube.Date.Year["2020"].December
])
\end{lstlisting}


==> listings/reference_january.tex <==
\begin{lstlisting}[caption={Referencing the January 2020 level member},label={lst:ref_jan}]
sales_cube.Date.Year["2020"].January
\end{lstlisting}


==> listings/reference_january_subscript.tex <==
\begin{lstlisting}[caption={Referencing a level member using the subscript syntax},label={lst:ref_subscript_syntax}]
sales_cube.Date.Year["2020"]["January"]
\end{lstlisting}


==> listings/restrict_suppliers_to_denmark.tex <==
\begin{lstlisting}[caption={Limit results to Danish suppliers},label={lst:almost_full_example}]
c = sales_cube
        .columns(sales_cube.Date.Year["2020"].children())
        .rows(sales_cube.Product.Category.members())
        .pages(sales_cube.Store.City.members())
        .where(sales_cube.Supplier.Nation == "Denmark")
\end{lstlisting}


==> listings/second_order_conversion.tex <==
\begin{lstlisting}[caption={Manipulating a cube further},label={lst:conv_cube_2}]
    c1 = c.columns(base_cube.Product.Name.members())
          .rows(base_cube.Date.Year["2020"].children())
\end{lstlisting}


==> listings/set_default_measure.tex <==
\begin{lstlisting}[caption={Setting the default measure},label={lst:setdefaultmeasure}]
sales_cube.set_default_measure(sales_cube.UnitSales)
\end{lstlisting}


==> listings/store_dimension_qb4olap.tex <==
\begin{minipage}{\linewidth}
\begin{lstlisting}[label={lst:store_dimension},caption={The store dimension in QB4OLAP}]
eg:store a qb:DimensionProperty .

eg:size a qb:AttributeProperty .

eg:store_address a qb4o:LevelProperty ;
    qb4o:hasAttribute eg:size ;
    qb4o:inDimension eg:store ;
    qb4o:parentLevel eg:store_city .

eg:store_city a qb4o:LevelProperty ;
    qb4o:inDimension eg:store ;
    qb4o:parentLevel eg:store_county .

eg:store_county a qb4o:LevelProperty ;
    qb4o:inDimension eg:store .

\end{lstlisting}
\end{minipage}


==> listings/using_unitsales_measure.tex <==
\begin{lstlisting}[caption={Using the \inlinecode{UnitSales} measure},label={lst:full_example}]
c = base_cube.columns(base_cube.Date.Year._2020.children())
             .rows(base_cube.Product.Category.members())
             .pages(base_cube.Store.City.members())
             .where(base_cube.Supplier.Nation="Denmark")
             .measures(base_cube.UnitSales)
\end{lstlisting}

